COIN: Communication-Aware In-Memory Acceleration for Graph Convolutional Networks

Graph convolutional networks (GCNs) have shown remarkable learning capabilities when processing graph-structured data found inherently in many application areas. GCNs distribute the outputs of neural networks embedded in each vertex over multiple iterations to take advantage of the relations captured by the underlying graphs. Consequently, they incur a significant amount of computation and irregular communication overheads, which call for GCN-specific hardware accelerators. To this end, this paper presents a communication-aware in-memory computing architecture (COIN) for GCN hardware acceleration. Besides accelerating the computation using custom compute elements (CE) and in-memory computing, COIN aims at minimizing the intra- and inter-CE communication in GCN operations to optimize the performance and energy efficiency. Experimental evaluations with widely used datasets show up to 105x improvement in energy consumption compared to state-of-the-art GCN accelerator.

==> files/acknowledgement.tex <==
\section{Acknowledgements}

This work was supported in part by C-BRIC, one of the six centers in JUMP, a Semiconductor Research Corporation program sponsored by DARPA, NSF~CAREER~Award CNS-1651624 and Semiconductor Research Corporation under task ID 2938.001.

\vspace{-3mm}

==> files/arch.tex <==
\section{Overview of Generated IMC Architecture}





==> files/discussion.tex <==
\section{Discussion and Conclusion}

==> files/noc_mapping.tex <==
\begin{figure}[b]
	\centering
% 	\vspace{-4mm}
	\includegraphics[width=1\columnwidth]{figures/conn_power.png}
% 	\vspace{-6mm}
	\caption{NoC optimization effectively reduces the power consumption because of its non-linear dependence on the mesh size. We obtain NoC power through BookSim~\cite{jiang2013detailed} simulations.} 
	\label{fig:conn_optim}
% 	\vspace{-4mm}
\end{figure}

% \section{Energy-Aware Optimization for NoC} \label{sec:interconnect}
\noindent\textbf{Energy-Aware Optimization for NoC: }
As a result of proposed area-aware optimization, the total number of tiles in an IMC architecture can be very high.
For example, DenseNet (100,24) requires 1,088 tiles~\cite{chen2018neurosim}. For such an architecture, one-to-one mapping of router to tile~\cite{kwon2017rethinking} will require a large number of NoC routers resulting in high power consumption, as shown in Figure~\ref{fig:conn_optim}.
Therefore, our proposed optimization framework minimizes energy consumption in NoC. 
% Therefore, Section~\ref{sec:sched} presents a technique to schedule the injection of activations and avoid congestion in the NoC.
%
%
% \subsection{Mapping Tiles to Routers} \label{sec:tile_to_router}

\noindent\textit{\underline{Mapping Tiles to Routers:}}
We first construct an objective function that represents the NoC energy consumption.
Let $n_k$ be the number of routers required for the $k^\mathrm{th}$ layer of the DNN.
The number of activations communicated between $n_k$ and $n_{k+1}$ routers is $I_k$. Hence, the number of activations between each source-destination pair is given by ${I_k}/{(n_k \times n_{k+1})}$.
The total amount of communication volume can be found by adding this across all K layers and routers:
%
\begin{equation} \label{eq:noc_obj}
    E(\mathbf{\bar{n}}) = \Big( \sum_{k=1}^{K-1} \frac{I_k}{n_k n_{k+1}} \Big) \Big( \sum_{k=1}^{K} n_k \Big)
\end{equation}
%
% This term is proportional to the total communication latency for the DNN.
This term is proportional to the total communication energy for the DNN assuming that all transactions have uniform size.
We minimize this objective function with an upper bound on the total number of routers, N as:
%
\begin{equation} \label{eq:constraints}
\begin{aligned}
& \underset{\mathbf{\bar{n}}}{\text{minimize}}
& & E(\mathbf{\bar{n}}) \\
& \text{subject to}
& & n_k \geq 1 ; k = 1, \ldots, K, \\
& & &\sum_{k=1}^{K} n_k < N.
\end{aligned}
\end{equation}
%
where the first constraint ensures that each layer of the DNN is associated with at least one router. N is a user defined constraint (input to the optimization framework) on the maximum number of routers in the IMC architecture.
At the end of this optimization, we obtain the number of routers needed for each layer ($n_k$) of the DNN.

% \subsection{Packet Scheduling in NoC}
\noindent\textit{\underline{Packet Scheduling in NoC:} }
% \label{sec:sched}
If the activations of a layer are injected into the NoC in the order of computation, there is a high possibility of congestion resulting in high communication latency in the NoC. 
Therefore, we propose a scheduling technique for the NoC to schedule the activations between two layers of the DNN.
\dnt{The scheduling technique is applied on top of the optimal tile to router mapped NoC.}
This scheduling technique provides a starting time for activations from each source to destination pair in the NoC.
Without loss of generality, we assume that all activations for a particular source-destination pair can be injected back-to-back.

Using the NoC topology and the routing algorithm, we first find the source-destination pairs which contend for the same link in the NoC.
We model each source-destination pair ($sd$) as an individual task.
The start time of the task corresponding to the pair $sd$ is denoted by $t_{sd}$ and the duration of the task equals to the number of packets for that pair ($n_{sd}$).
Next, 
% we formulate constraints to avoid any contention between different tasks.
we put constraints on the start time of each task so that there is no contention between two transactions contending for the same link.
The set of all tasks is denoted by $\mathcal{T}$ and the set of all non-overlapping tasks is denoted by $\mathcal{C}$.
\eqref{eq:sched_eqn} shows formulation of the non-overlap constraint, where the start time of two tasks is separated by the duration.
Furthermore, the start time of all tasks are integers and greater than zero.
We add one terminal task with the constraint that the start time of the terminal task ($t_{terminal}$) is greater than the start time of any of the source-destination pairs.
% Minimizing $t_{terminal}$ corresponds to minimizing the total transaction time for all source-destination pairs.
% Therefore, 
We minimize $t_{terminal}$ to obtain the optimal schedule for all source-destination pairs.
% These schedules are implemented as a look-up table at each router of the NoC.
%
\begin{equation} \label{eq:sched_eqn}
\begin{aligned}
& \text{minimize} & & t_{terminal} \\
& \text{subject to}
& & t_{mn} > t_{pq} + n_{pq} \lor t_{pq} > t_{mn} + n_{pq}, \\
& & & \forall t_{mn}, t_{pq} \in \mathcal{C}, \\
& & & t_{xy} \geq 0, \forall t_{xy} \in \mathcal{T}\\
& & & t_{terminal} > t_{xy} + n_{xy}, \forall t_{xy} \in \mathcal{T}.
\end{aligned}
\end{equation}
